Unifying Causal Inference and Reinforcement Learning using Higher-Order Category Theory

We present a unified formalism for structure discovery of causal models and predictive state representation (PSR) models in reinforcement learning (RL) using higher-order category theory. Specifically, we model structure discovery in both settings using simplicial objects, contravariant functors from the category of ordinal numbers into any category. Fragments of causal models that are equivalent under conditional independence -- defined as causal horns -- as well as subsequences of potential tests in a predictive state representation -- defined as predictive horns -- are both special cases of horns of a simplicial object, subsets resulting from the removal of the interior and the face opposite a particular vertex. Latent structure discovery in both settings involve the same fundamental mathematical problem of finding extensions of horns of simplicial objects through solving lifting problems in commutative diagrams, and exploiting weak homotopies that define higher-order symmetries. Solutions to the problem of filling "inner" vs "outer" horns leads to various notions of higher-order categories, including weak Kan complexes and quasicategories. We define the abstract problem of structure discovery in both settings in terms of adjoint functors between the category of universal causal models or universal decision models and its simplicial object representation.

==> Unifying Causal Inference and RL Arxiv Submission/output.tex <==
\begin{thebibliography}{42}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[MacLane(1971)]{maclane:71}
Saunders MacLane.
\newblock \emph{Categories for the Working Mathematician}.
\newblock Springer-Verlag, New York, 1971.
\newblock Graduate Texts in Mathematics, Vol. 5.

\bibitem[Pearl(1989)]{pearl:bnets-book}
Judea Pearl.
\newblock \emph{Probabilistic reasoning in intelligent systems - networks of
  plausible inference}.
\newblock Morgan Kaufmann series in representation and reasoning. Morgan
  Kaufmann, 1989.

\bibitem[Pearl(2009)]{pearl:causalitybook}
Judea Pearl.
\newblock \emph{Causality: Models, Reasoning and Inference}.
\newblock Cambridge University Press, USA, 2nd edition, 2009.
\newblock ISBN 052189560X.

\bibitem[Studeny(2010)]{studeny2010probabilistic}
M.~Studeny.
\newblock \emph{Probabilistic Conditional Independence Structures}.
\newblock Information Science and Statistics. Springer London, 2010.
\newblock ISBN 9781849969482.
\newblock URL \url{https://books.google.com.gi/books?id=bGFRcgAACAAJ}.

\bibitem[Matus(1995)]{matus}
F.~Matus.
\newblock Conditional independence among four random variables.
\newblock \emph{Combinatorics, Probability and Computing}, 5:\penalty0
  407--417, 1995.

\bibitem[Dawid(2001)]{DBLP:journals/amai/Dawid01}
A.~Philip Dawid.
\newblock Separoids: {A} mathematical framework for conditional independence
  and irrelevance.
\newblock \emph{Ann. Math. Artif. Intell.}, 32\penalty0 (1-4):\penalty0
  335--372, 2001.
\newblock \doi{10.1023/A:1016734104787}.
\newblock URL \url{https://doi.org/10.1023/A:1016734104787}.

\bibitem[Dawid(2010)]{DBLP:journals/jmlr/Dawid10}
A.~Philip Dawid.
\newblock Beware of the dag!
\newblock In Isabelle Guyon, Dominik Janzing, and Bernhard Sch{\"{o}}lkopf,
  editors, \emph{Causality: Objectives and Assessment {(NIPS} 2008 Workshop),
  Whistler, Canada, December 12, 2008}, volume~6 of \emph{{JMLR} Proceedings},
  pages 59--86. JMLR.org, 2010.
\newblock URL \url{http://proceedings.mlr.press/v6/dawid10a.html}.

\bibitem[Lauritzen and Richardson(2002)]{lauritzen:chain}
Steffen~L. Lauritzen and Thomas~S. Richardson.
\newblock Chain graph models and their causal interpretations.
\newblock \emph{Journal of the Royal Statistical Society: Series B (Statistical
  Methodology)}, 64\penalty0 (3):\penalty0 321--348, 2002.
\newblock \doi{https://doi.org/10.1111/1467-9868.00340}.
\newblock URL
  \url{https://rss.onlinelibrary.wiley.com/doi/abs/10.1111/1467-9868.00340}.

\bibitem[Evans(2018)]{mdag}
Robin~J. Evans.
\newblock {Margins of discrete Bayesian networks}.
\newblock \emph{The Annals of Statistics}, 46\penalty0 (6A):\penalty0 2623 --
  2656, 2018.
\newblock \doi{10.1214/17-AOS1631}.
\newblock URL \url{https://doi.org/10.1214/17-AOS1631}.

\bibitem[Forré and Mooij(2017)]{hedge}
Patrick Forré and Joris~M. Mooij.
\newblock Markov properties for graphical models with cycles and latent
  variables, 2017.

\bibitem[Amini et~al.(2022)Amini, Aragam, and Zhou]{amini}
Arash~A. Amini, Bryon Aragam, and Qing Zhou.
\newblock A non-graphical representation of conditional independence via the
  neighbourhood lattice, 2022.
\newblock URL \url{https://arxiv.org/abs/2206.05829}.

\bibitem[Heymann et~al.(2020)Heymann, de~Lara, and Chancelier]{cif}
Bejamin Heymann, Michel de~Lara, and Jean-Philippe Chancelier.
\newblock Causal information with information fields.
\newblock In \emph{Neural Inforamtion Processing Systems Workshop on Causal
  Discovery and Causality-inspired Machine Learning}, 2020.

\bibitem[Sadeghi(2017)]{sadeghi}
Kayvan Sadeghi.
\newblock Faithfulness of probability distributions and graphs.
\newblock 2017.
\newblock \doi{10.48550/ARXIV.1701.08366}.
\newblock URL \url{https://arxiv.org/abs/1701.08366}.

\bibitem[Richter(2020)]{richter2020categories}
B.~Richter.
\newblock \emph{From Categories to Homotopy Theory}.
\newblock Cambridge Studies in Advanced Mathematics. Cambridge University
  Press, 2020.
\newblock ISBN 9781108479622.
\newblock URL \url{https://books.google.com/books?id=pnzUDwAAQBAJ}.

\bibitem[Riehl(2017)]{riehl2017category}
E.~Riehl.
\newblock \emph{Category Theory in Context}.
\newblock Aurora: Dover Modern Math Originals. Dover Publications, 2017.
\newblock ISBN 9780486820804.
\newblock URL \url{https://books.google.com/books?id=6B9MDgAAQBAJ}.

\bibitem[Bouckaert et~al.(2010)Bouckaert, Hemmecke, Lindner, and
  Studen\'{y}]{bouckaert}
Remco Bouckaert, Raymond Hemmecke, Silvia Lindner, and Milan Studen\'{y}.
\newblock Efficient algorithms for conditional independence inference.
\newblock \emph{J. Mach. Learn. Res.}, 11:\penalty0 3453–3479, dec 2010.
\newblock ISSN 1532-4435.

\bibitem[Sam and Snowden(2016)]{Sam_2016}
Steven Sam and Andrew Snowden.
\newblock Gr\"obner methods for representations of combinatorial categories.
\newblock \emph{Journal of the American Mathematical Society}, 30\penalty0
  (1):\penalty0 159--203, mar 2016.
\newblock \doi{10.1090/jams/859}.
\newblock URL \url{https://doi.org/10.1090%2Fjams%2F859}.

\bibitem[Baez and Stay(2010)]{Baez_2010}
J.~Baez and M.~Stay.
\newblock Physics, topology, logic and computation: A rosetta stone.
\newblock In \emph{New Structures for Physics}, pages 95--172. Springer Berlin
  Heidelberg, 2010.
\newblock \doi{10.1007/978-3-642-12821-9_2}.
\newblock URL \url{https://doi.org/10.1007%2F978-3-642-12821-9_2}.

\bibitem[MacLane and leke Moerdijk(1994)]{maclane:sheaves}
Saunders MacLane and leke Moerdijk.
\newblock \emph{Sheaves in Geometry and Logic: A First Introduction to Topos
  Theory}.
\newblock Springer, 1994.

\bibitem[Lewis(1972)]{mobius}
D.~C. Lewis.
\newblock {A generalized Möbius inversion formula}.
\newblock \emph{Bulletin of the American Mathematical Society}, 78\penalty0
  (4):\penalty0 558 -- 561, 1972.
\newblock \doi{bams/1183533895}.
\newblock URL \url{https://doi.org/}.

\bibitem[Mahadevan(2022)]{sm:uc}
Sridhar Mahadevan.
\newblock On the universality of diagrams for causal inference and the causal
  reproducing property, 2022.
\newblock URL \url{https://arxiv.org/abs/2207.02917}.

\bibitem[Joyal et~al.(1996)Joyal, Nielsen, and Winskel]{JOYAL1996164}
André Joyal, Mogens Nielsen, and Glynn Winskel.
\newblock Bisimulation from open maps.
\newblock \emph{Information and Computation}, 127\penalty0 (2):\penalty0
  164--185, 1996.
\newblock ISSN 0890-5401.
\newblock \doi{https://doi.org/10.1006/inco.1996.0057}.
\newblock URL
  \url{https://www.sciencedirect.com/science/article/pii/S0890540196900577}.

\bibitem[Fong and Spivak(2018)]{fong2018seven}
Brendan Fong and David~I Spivak.
\newblock \emph{Seven Sketches in Compositionality: An Invitation to Applied
  Category Theory}.
\newblock 2018.
\newblock URL \url{http://arxiv.org/abs/1803.05316}.
\newblock cite arxiv:1803.05316Comment: 341+xii pages.

\bibitem[Andersson et~al.(1997)Andersson, Madigan, Perlman, and
  Triggs]{DBLP:journals/amai/AnderssonMPT97}
Steen~A. Andersson, David Madigan, Michael~D. Perlman, and Christopher~M.
  Triggs.
\newblock A graphical characterization of lattice conditional independence
  models.
\newblock \emph{Ann. Math. Artif. Intell.}, 21\penalty0 (1):\penalty0 27--50,
  1997.
\newblock \doi{10.1023/A:1018901032102}.
\newblock URL \url{https://doi.org/10.1023/A:1018901032102}.

\bibitem[Hibi(1987)]{hibi1987distributive}
Takayuki Hibi.
\newblock Distributive lattices, affine semigroup rings and algebras with
  straightening laws.
\newblock \emph{Commutative algebra and combinatorics}, 11:\penalty0 93--109,
  1987.

\bibitem[Beerenwinkel et~al.(2007)Beerenwinkel, Eriksson, and Sturmfels]{cbn}
Niko Beerenwinkel, Nicholas Eriksson, and Bernd Sturmfels.
\newblock {Conjunctive Bayesian networks}.
\newblock \emph{Bernoulli}, 13\penalty0 (4):\penalty0 893 -- 909, 2007.
\newblock \doi{10.3150/07-BEJ6133}.
\newblock URL \url{https://doi.org/10.3150/07-BEJ6133}.

\bibitem[Geiger et~al.(2006)Geiger, Meek, and Sturmfels]{Geiger_2006}
Dan Geiger, Christopher Meek, and Bernd Sturmfels.
\newblock On the toric algebra of graphical models.
\newblock \emph{The Annals of Statistics}, 34\penalty0 (3), jun 2006.
\newblock \doi{10.1214/009053606000000263}.
\newblock URL \url{https://doi.org/10.1214%2F009053606000000263}.

\bibitem[Lurie(2006)]{lurie}
Jacob Lurie.
\newblock Higher topos theory, 2006.
\newblock URL \url{https://arxiv.org/abs/math/0608040}.

\bibitem[Fong(2012)]{fong:ms}
Brendan Fong.
\newblock Causal theories: A categorical perspective on bayesian networks,
  2012.

\bibitem[Witsenhausen(1975)]{witsenhausen:1975}
H.~S. Witsenhausen.
\newblock The intrinsic model for discrete stochastic control: Some open
  problems.
\newblock In A.~Bensoussan and J.~L. Lions, editors, \emph{Control Theory,
  Numerical Methods and Computer Systems Modelling}, pages 322--335, Berlin,
  Heidelberg, 1975. Springer Berlin Heidelberg.
\newblock ISBN 978-3-642-46317-4.

\bibitem[Mahadevan(2021)]{sm:homotopy}
Sridhar Mahadevan.
\newblock Causal homotopy, 2021.
\newblock URL \url{https://arxiv.org/abs/2112.01847}.

\bibitem[Andersson et~al.(1996)Andersson, Madigan, and
  Perlman]{DBLP:conf/uai/AnderssonMP96}
Steen~A. Andersson, David Madigan, and Michael~D. Perlman.
\newblock An alternative markov property for chain graphs.
\newblock In Eric Horvitz and Finn~Verner Jensen, editors, \emph{{UAI} '96:
  Proceedings of the Twelfth Annual Conference on Uncertainty in Artificial
  Intelligence, Reed College, Portland, Oregon, USA, August 1-4, 1996}, pages
  40--48. Morgan Kaufmann, 1996.
\newblock URL
  \url{https://dslpitt.org/uai/displayArticleDetails.jsp?mmnu=1\&smnu=2\&article\_id=350\&proceeding\_id=12}.

\bibitem[Bradley et~al.(2022)Bradley, Terilla, and Vlassopoulos]{Bradley_2022}
Tai-Danae Bradley, John Terilla, and Yiannis Vlassopoulos.
\newblock An enriched category theory of language: From syntax to semantics.
\newblock \emph{La Matematica}, mar 2022.
\newblock \doi{10.1007/s44007-022-00021-2}.
\newblock URL \url{https://doi.org/10.1007\%2Fs44007-022-00021-2}.

\bibitem[Beerenwinkel et~al.(2006)Beerenwinkel, Eriksson, and
  Sturmfels]{BEERENWINKEL2006409}
Niko Beerenwinkel, Nicholas Eriksson, and Bernd Sturmfels.
\newblock Evolution on distributive lattices.
\newblock \emph{Journal of Theoretical Biology}, 242\penalty0 (2):\penalty0
  409--420, 2006.
\newblock ISSN 0022-5193.
\newblock \doi{https://doi.org/10.1016/j.jtbi.2006.03.013}.
\newblock URL
  \url{https://www.sciencedirect.com/science/article/pii/S0022519306001159}.

\bibitem[Censi(2015)]{censi}
Andrea Censi.
\newblock A mathematical theory of co-design, 2015.
\newblock URL \url{https://arxiv.org/abs/1512.08055}.

\bibitem[Fong(2015)]{cospans}
Brendan Fong.
\newblock Decorated cospans.
\newblock 2015.
\newblock \doi{10.48550/ARXIV.1502.00872}.
\newblock URL \url{https://arxiv.org/abs/1502.00872}.

\bibitem[Leinster(2003)]{higher-operads}
Tom Leinster.
\newblock Higher operads, higher categories, 2003.
\newblock URL \url{https://arxiv.org/abs/math/0305049}.

\bibitem[Spivak(2013)]{operads-db}
David~I. Spivak.
\newblock The operad of wiring diagrams: formalizing a graphical language for
  databases, recursion, and plug-and-play circuits, 2013.
\newblock URL \url{https://arxiv.org/abs/1305.0297}.

\bibitem[Joyal et~al.(1993)Joyal, Nielsen, and
  Winskel]{DBLP:conf/lics/JoyalNW93}
Andr{\'{e}} Joyal, Mogens Nielsen, and Glynn Winskel.
\newblock Bisimulation and open maps.
\newblock In \emph{Proceedings of the Eighth Annual Symposium on Logic in
  Computer Science {(LICS} '93), Montreal, Canada, June 19-23, 1993}, pages
  418--427. {IEEE} Computer Society, 1993.
\newblock \doi{10.1109/LICS.1993.287566}.
\newblock URL \url{https://doi.org/10.1109/LICS.1993.287566}.

\bibitem[Cattani and Winskel(2005)]{bisim}
Gian~Luca Cattani and Glynn Winskel.
\newblock Profunctors, open maps and bisimulation.
\newblock \emph{Math. Struct. Comput. Sci.}, 15\penalty0 (3):\penalty0
  553--614, 2005.
\newblock \doi{10.1017/S0960129505004718}.
\newblock URL \url{https://doi.org/10.1017/S0960129505004718}.

\bibitem[Goldblatt(2006)]{goldblatt:topos}
Robert Goldblatt.
\newblock \emph{Topoi: The Categorial Analysis of Logic}.
\newblock Dover Press, 2006.

\bibitem[Johnstone(2002)]{Johnstone:592033}
Peter~T Johnstone.
\newblock \emph{{Sketches of an elephant: a Topos theory compendium}}.
\newblock Oxford logic guides. Oxford Univ. Press, New York, NY, 2002.
\newblock URL \url{https://cds.cern.ch/record/592033}.

\end{thebibliography}


==> output.tex <==
\begin{thebibliography}{42}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[MacLane(1971)]{maclane:71}
Saunders MacLane.
\newblock \emph{Categories for the Working Mathematician}.
\newblock Springer-Verlag, New York, 1971.
\newblock Graduate Texts in Mathematics, Vol. 5.

\bibitem[Pearl(1989)]{pearl:bnets-book}
Judea Pearl.
\newblock \emph{Probabilistic reasoning in intelligent systems - networks of
  plausible inference}.
\newblock Morgan Kaufmann series in representation and reasoning. Morgan
  Kaufmann, 1989.

\bibitem[Pearl(2009)]{pearl:causalitybook}
Judea Pearl.
\newblock \emph{Causality: Models, Reasoning and Inference}.
\newblock Cambridge University Press, USA, 2nd edition, 2009.
\newblock ISBN 052189560X.

\bibitem[Studeny(2010)]{studeny2010probabilistic}
M.~Studeny.
\newblock \emph{Probabilistic Conditional Independence Structures}.
\newblock Information Science and Statistics. Springer London, 2010.
\newblock ISBN 9781849969482.
\newblock URL \url{https://books.google.com.gi/books?id=bGFRcgAACAAJ}.

\bibitem[Matus(1995)]{matus}
F.~Matus.
\newblock Conditional independence among four random variables.
\newblock \emph{Combinatorics, Probability and Computing}, 5:\penalty0
  407--417, 1995.

\bibitem[Dawid(2001)]{DBLP:journals/amai/Dawid01}
A.~Philip Dawid.
\newblock Separoids: {A} mathematical framework for conditional independence
  and irrelevance.
\newblock \emph{Ann. Math. Artif. Intell.}, 32\penalty0 (1-4):\penalty0
  335--372, 2001.
\newblock \doi{10.1023/A:1016734104787}.
\newblock URL \url{https://doi.org/10.1023/A:1016734104787}.

\bibitem[Dawid(2010)]{DBLP:journals/jmlr/Dawid10}
A.~Philip Dawid.
\newblock Beware of the dag!
\newblock In Isabelle Guyon, Dominik Janzing, and Bernhard Sch{\"{o}}lkopf,
  editors, \emph{Causality: Objectives and Assessment {(NIPS} 2008 Workshop),
  Whistler, Canada, December 12, 2008}, volume~6 of \emph{{JMLR} Proceedings},
  pages 59--86. JMLR.org, 2010.
\newblock URL \url{http://proceedings.mlr.press/v6/dawid10a.html}.

\bibitem[Lauritzen and Richardson(2002)]{lauritzen:chain}
Steffen~L. Lauritzen and Thomas~S. Richardson.
\newblock Chain graph models and their causal interpretations.
\newblock \emph{Journal of the Royal Statistical Society: Series B (Statistical
  Methodology)}, 64\penalty0 (3):\penalty0 321--348, 2002.
\newblock \doi{https://doi.org/10.1111/1467-9868.00340}.
\newblock URL
  \url{https://rss.onlinelibrary.wiley.com/doi/abs/10.1111/1467-9868.00340}.

\bibitem[Evans(2018)]{mdag}
Robin~J. Evans.
\newblock {Margins of discrete Bayesian networks}.
\newblock \emph{The Annals of Statistics}, 46\penalty0 (6A):\penalty0 2623 --
  2656, 2018.
\newblock \doi{10.1214/17-AOS1631}.
\newblock URL \url{https://doi.org/10.1214/17-AOS1631}.

\bibitem[Forré and Mooij(2017)]{hedge}
Patrick Forré and Joris~M. Mooij.
\newblock Markov properties for graphical models with cycles and latent
  variables, 2017.

\bibitem[Amini et~al.(2022)Amini, Aragam, and Zhou]{amini}
Arash~A. Amini, Bryon Aragam, and Qing Zhou.
\newblock A non-graphical representation of conditional independence via the
  neighbourhood lattice, 2022.
\newblock URL \url{https://arxiv.org/abs/2206.05829}.

\bibitem[Heymann et~al.(2020)Heymann, de~Lara, and Chancelier]{cif}
Bejamin Heymann, Michel de~Lara, and Jean-Philippe Chancelier.
\newblock Causal information with information fields.
\newblock In \emph{Neural Inforamtion Processing Systems Workshop on Causal
  Discovery and Causality-inspired Machine Learning}, 2020.

\bibitem[Sadeghi(2017)]{sadeghi}
Kayvan Sadeghi.
\newblock Faithfulness of probability distributions and graphs.
\newblock 2017.
\newblock \doi{10.48550/ARXIV.1701.08366}.
\newblock URL \url{https://arxiv.org/abs/1701.08366}.

\bibitem[Richter(2020)]{richter2020categories}
B.~Richter.
\newblock \emph{From Categories to Homotopy Theory}.
\newblock Cambridge Studies in Advanced Mathematics. Cambridge University
  Press, 2020.
\newblock ISBN 9781108479622.
\newblock URL \url{https://books.google.com/books?id=pnzUDwAAQBAJ}.

\bibitem[Riehl(2017)]{riehl2017category}
E.~Riehl.
\newblock \emph{Category Theory in Context}.
\newblock Aurora: Dover Modern Math Originals. Dover Publications, 2017.
\newblock ISBN 9780486820804.
\newblock URL \url{https://books.google.com/books?id=6B9MDgAAQBAJ}.

\bibitem[Bouckaert et~al.(2010)Bouckaert, Hemmecke, Lindner, and
  Studen\'{y}]{bouckaert}
Remco Bouckaert, Raymond Hemmecke, Silvia Lindner, and Milan Studen\'{y}.
\newblock Efficient algorithms for conditional independence inference.
\newblock \emph{J. Mach. Learn. Res.}, 11:\penalty0 3453–3479, dec 2010.
\newblock ISSN 1532-4435.

\bibitem[Sam and Snowden(2016)]{Sam_2016}
Steven Sam and Andrew Snowden.
\newblock Gr\"obner methods for representations of combinatorial categories.
\newblock \emph{Journal of the American Mathematical Society}, 30\penalty0
  (1):\penalty0 159--203, mar 2016.
\newblock \doi{10.1090/jams/859}.
\newblock URL \url{https://doi.org/10.1090%2Fjams%2F859}.

\bibitem[Baez and Stay(2010)]{Baez_2010}
J.~Baez and M.~Stay.
\newblock Physics, topology, logic and computation: A rosetta stone.
\newblock In \emph{New Structures for Physics}, pages 95--172. Springer Berlin
  Heidelberg, 2010.
\newblock \doi{10.1007/978-3-642-12821-9_2}.
\newblock URL \url{https://doi.org/10.1007%2F978-3-642-12821-9_2}.

\bibitem[MacLane and leke Moerdijk(1994)]{maclane:sheaves}
Saunders MacLane and leke Moerdijk.
\newblock \emph{Sheaves in Geometry and Logic: A First Introduction to Topos
  Theory}.
\newblock Springer, 1994.

\bibitem[Lewis(1972)]{mobius}
D.~C. Lewis.
\newblock {A generalized Möbius inversion formula}.
\newblock \emph{Bulletin of the American Mathematical Society}, 78\penalty0
  (4):\penalty0 558 -- 561, 1972.
\newblock \doi{bams/1183533895}.
\newblock URL \url{https://doi.org/}.

\bibitem[Mahadevan(2022)]{sm:uc}
Sridhar Mahadevan.
\newblock On the universality of diagrams for causal inference and the causal
  reproducing property, 2022.
\newblock URL \url{https://arxiv.org/abs/2207.02917}.

\bibitem[Joyal et~al.(1996)Joyal, Nielsen, and Winskel]{JOYAL1996164}
André Joyal, Mogens Nielsen, and Glynn Winskel.
\newblock Bisimulation from open maps.
\newblock \emph{Information and Computation}, 127\penalty0 (2):\penalty0
  164--185, 1996.
\newblock ISSN 0890-5401.
\newblock \doi{https://doi.org/10.1006/inco.1996.0057}.
\newblock URL
  \url{https://www.sciencedirect.com/science/article/pii/S0890540196900577}.

\bibitem[Fong and Spivak(2018)]{fong2018seven}
Brendan Fong and David~I Spivak.
\newblock \emph{Seven Sketches in Compositionality: An Invitation to Applied
  Category Theory}.
\newblock 2018.
\newblock URL \url{http://arxiv.org/abs/1803.05316}.
\newblock cite arxiv:1803.05316Comment: 341+xii pages.

\bibitem[Andersson et~al.(1997)Andersson, Madigan, Perlman, and
  Triggs]{DBLP:journals/amai/AnderssonMPT97}
Steen~A. Andersson, David Madigan, Michael~D. Perlman, and Christopher~M.
  Triggs.
\newblock A graphical characterization of lattice conditional independence
  models.
\newblock \emph{Ann. Math. Artif. Intell.}, 21\penalty0 (1):\penalty0 27--50,
  1997.
\newblock \doi{10.1023/A:1018901032102}.
\newblock URL \url{https://doi.org/10.1023/A:1018901032102}.

\bibitem[Hibi(1987)]{hibi1987distributive}
Takayuki Hibi.
\newblock Distributive lattices, affine semigroup rings and algebras with
  straightening laws.
\newblock \emph{Commutative algebra and combinatorics}, 11:\penalty0 93--109,
  1987.

\bibitem[Beerenwinkel et~al.(2007)Beerenwinkel, Eriksson, and Sturmfels]{cbn}
Niko Beerenwinkel, Nicholas Eriksson, and Bernd Sturmfels.
\newblock {Conjunctive Bayesian networks}.
\newblock \emph{Bernoulli}, 13\penalty0 (4):\penalty0 893 -- 909, 2007.
\newblock \doi{10.3150/07-BEJ6133}.
\newblock URL \url{https://doi.org/10.3150/07-BEJ6133}.

\bibitem[Geiger et~al.(2006)Geiger, Meek, and Sturmfels]{Geiger_2006}
Dan Geiger, Christopher Meek, and Bernd Sturmfels.
\newblock On the toric algebra of graphical models.
\newblock \emph{The Annals of Statistics}, 34\penalty0 (3), jun 2006.
\newblock \doi{10.1214/009053606000000263}.
\newblock URL \url{https://doi.org/10.1214%2F009053606000000263}.

\bibitem[Lurie(2006)]{lurie}
Jacob Lurie.
\newblock Higher topos theory, 2006.
\newblock URL \url{https://arxiv.org/abs/math/0608040}.

\bibitem[Fong(2012)]{fong:ms}
Brendan Fong.
\newblock Causal theories: A categorical perspective on bayesian networks,
  2012.

\bibitem[Witsenhausen(1975)]{witsenhausen:1975}
H.~S. Witsenhausen.
\newblock The intrinsic model for discrete stochastic control: Some open
  problems.
\newblock In A.~Bensoussan and J.~L. Lions, editors, \emph{Control Theory,
  Numerical Methods and Computer Systems Modelling}, pages 322--335, Berlin,
  Heidelberg, 1975. Springer Berlin Heidelberg.
\newblock ISBN 978-3-642-46317-4.

\bibitem[Mahadevan(2021)]{sm:homotopy}
Sridhar Mahadevan.
\newblock Causal homotopy, 2021.
\newblock URL \url{https://arxiv.org/abs/2112.01847}.

\bibitem[Andersson et~al.(1996)Andersson, Madigan, and
  Perlman]{DBLP:conf/uai/AnderssonMP96}
Steen~A. Andersson, David Madigan, and Michael~D. Perlman.
\newblock An alternative markov property for chain graphs.
\newblock In Eric Horvitz and Finn~Verner Jensen, editors, \emph{{UAI} '96:
  Proceedings of the Twelfth Annual Conference on Uncertainty in Artificial
  Intelligence, Reed College, Portland, Oregon, USA, August 1-4, 1996}, pages
  40--48. Morgan Kaufmann, 1996.
\newblock URL
  \url{https://dslpitt.org/uai/displayArticleDetails.jsp?mmnu=1\&smnu=2\&article\_id=350\&proceeding\_id=12}.

\bibitem[Bradley et~al.(2022)Bradley, Terilla, and Vlassopoulos]{Bradley_2022}
Tai-Danae Bradley, John Terilla, and Yiannis Vlassopoulos.
\newblock An enriched category theory of language: From syntax to semantics.
\newblock \emph{La Matematica}, mar 2022.
\newblock \doi{10.1007/s44007-022-00021-2}.
\newblock URL \url{https://doi.org/10.1007\%2Fs44007-022-00021-2}.

\bibitem[Beerenwinkel et~al.(2006)Beerenwinkel, Eriksson, and
  Sturmfels]{BEERENWINKEL2006409}
Niko Beerenwinkel, Nicholas Eriksson, and Bernd Sturmfels.
\newblock Evolution on distributive lattices.
\newblock \emph{Journal of Theoretical Biology}, 242\penalty0 (2):\penalty0
  409--420, 2006.
\newblock ISSN 0022-5193.
\newblock \doi{https://doi.org/10.1016/j.jtbi.2006.03.013}.
\newblock URL
  \url{https://www.sciencedirect.com/science/article/pii/S0022519306001159}.

\bibitem[Censi(2015)]{censi}
Andrea Censi.
\newblock A mathematical theory of co-design, 2015.
\newblock URL \url{https://arxiv.org/abs/1512.08055}.

\bibitem[Fong(2015)]{cospans}
Brendan Fong.
\newblock Decorated cospans.
\newblock 2015.
\newblock \doi{10.48550/ARXIV.1502.00872}.
\newblock URL \url{https://arxiv.org/abs/1502.00872}.

\bibitem[Leinster(2003)]{higher-operads}
Tom Leinster.
\newblock Higher operads, higher categories, 2003.
\newblock URL \url{https://arxiv.org/abs/math/0305049}.

\bibitem[Spivak(2013)]{operads-db}
David~I. Spivak.
\newblock The operad of wiring diagrams: formalizing a graphical language for
  databases, recursion, and plug-and-play circuits, 2013.
\newblock URL \url{https://arxiv.org/abs/1305.0297}.

\bibitem[Joyal et~al.(1993)Joyal, Nielsen, and
  Winskel]{DBLP:conf/lics/JoyalNW93}
Andr{\'{e}} Joyal, Mogens Nielsen, and Glynn Winskel.
\newblock Bisimulation and open maps.
\newblock In \emph{Proceedings of the Eighth Annual Symposium on Logic in
  Computer Science {(LICS} '93), Montreal, Canada, June 19-23, 1993}, pages
  418--427. {IEEE} Computer Society, 1993.
\newblock \doi{10.1109/LICS.1993.287566}.
\newblock URL \url{https://doi.org/10.1109/LICS.1993.287566}.

\bibitem[Cattani and Winskel(2005)]{bisim}
Gian~Luca Cattani and Glynn Winskel.
\newblock Profunctors, open maps and bisimulation.
\newblock \emph{Math. Struct. Comput. Sci.}, 15\penalty0 (3):\penalty0
  553--614, 2005.
\newblock \doi{10.1017/S0960129505004718}.
\newblock URL \url{https://doi.org/10.1017/S0960129505004718}.

\bibitem[Goldblatt(2006)]{goldblatt:topos}
Robert Goldblatt.
\newblock \emph{Topoi: The Categorial Analysis of Logic}.
\newblock Dover Press, 2006.

\bibitem[Johnstone(2002)]{Johnstone:592033}
Peter~T Johnstone.
\newblock \emph{{Sketches of an elephant: a Topos theory compendium}}.
\newblock Oxford logic guides. Oxford Univ. Press, New York, NY, 2002.
\newblock URL \url{https://cds.cern.ch/record/592033}.

\end{thebibliography}

